Chronicling the Host Galaxy Properties of the Remarkable Repeating FRB 20201124A

We present the Australian Square Kilometre Array Pathfinder (ASKAP) localization and follow-up observations of the host galaxy of the repeating fast radio burst (FRB) source, FRB20201124A, the fifth such extragalactic repeating FRB with an identified host. From spectroscopic observations using the 6.5-m MMT Observatory, we derive a redshift of $z=0.0979 \pm 0.0001$, a star formation rate inferred from H$\alpha$ emission of SFR(H$\alpha$) $\approx 2.1 M_{\odot}$ yr$^{-1}$, and a gas-phase metallicity of 12+log(O/H)$\approx 9.0$. By jointly modeling the 12-filter optical-mid-infrared (MIR) photometry and spectroscopy of the host, we infer a median stellar mass of $\approx 2 \times 10^{10} M_{\odot}$, internal dust extinction of $A_V\approx 1-1.5$ mag, and a mass-weighted stellar population age of $\approx 5-6$ Gyr. Connecting these data to the radio and X-ray observations, we cannot reconcile the broad-band behavior with strong AGN activity and instead attribute the dominant source of persistent radio emission to star formation, likely originating from the circumnuclear region of the host. The modeling also indicates a hot dust component contributing to the MIR luminosity at a level of $\approx 10-30\%$. We model the host galaxy's star formation and mass assembly histories, finding that the host assembled $>90\%$ of its mass by 1 Gyr ago and exhibited a fairly constant SFR for most of its existence, with no clear evidence of past star-burst activity.

==> FRB 201124A host/affiliation.tex <==
\newcommand{\NU}{\affiliation{Center for Interdisciplinary Exploration and Research in Astrophysics (CIERA) and Department of Physics and Astronomy, Northwestern University, Evanston, IL 60208, USA}}

\newcommand{\Purdue}{\affiliation{Purdue University, 
Department of Physics and Astronomy, 525 Northwestern Avenue, West Lafayette, IN 47907, USA}}

\newcommand{\CfA}{\affiliation{Center for Astrophysics\:$|$\:Harvard \& Smithsonian, 60 Garden St. Cambridge, MA 02138, USA}}

\newcommand{\UCSC}{\affiliation{Department of Astronomy and Astrophysics, University of California, Santa Cruz, CA 95064, USA}}

\newcommand{\IS}{\affiliation{Centre for Astrophysics and Cosmology, Science Institute, University of Iceland, Dunhagi 5, 107 Reykjav\'ik, Iceland}}

\newcommand{\DAWN}{\affiliation{Cosmic Dawn Center (DAWN), Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2100 Copenhagen \O, Denmark}}

\newcommand{\PUCV}{\affiliation{Instituto de F\'isica, Pontificia Universidad Cat\'olica de Valpara\'iso, Casilla 4059, Valpara\'iso, Chile}}

\newcommand{\IPMU}{\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU), 5-1-5 Kashiwanoha, Kashiwa, 277-8583, Japan}}

\newcommand{\PSU}{\affiliation{Department of Astronomy \& Astrophysics, The Pennsylvania State University, University Park, PA 16802, USA}}

\newcommand{\ICDS}{\affiliation{Institute for Computational \& Data Sciences, The Pennsylvania State University, University Park, PA, USA}}

\newcommand{\IGC}{\affiliation{Institute for Gravitation and the Cosmos, The Pennsylvania State University, University Park, PA 16802, USA}}

\newcommand{\Swin}{\affiliation{ Centre for Astrophysics and Supercomputing, Swinburne University of Technology, Hawthorn, VIC, 3122, Australia}}

\newcommand{\Curtin}{\affiliation{ International Centre for Radio Astronomy Research, Curtin University, Bentley, WA 6102, Australia}}

\newcommand{\MQ}{\affiliation{Department of Physics \& Astronomy, Macquarie University, NSW 2109, Australia}}

\newcommand{\MQAAAstro}{\affiliation{Macquarie University Research Centre for Astronomy, Astrophysics \& Astrophotonics, Sydney, NSW 2109, Australia}}

\newcommand{\CSIRO}{\affiliation{CSIRO, Space and Astronomy, PO Box 76, Epping NSW 1710 Australia}}

==> FRB 201124A host/authors_frb201124a.tex <==
\author[0000-0002-7374-935X]{Wen-fai Fong}
\NU

\author[0000-0002-9363-8606]{Yuxin Dong}
\NU\Purdue

\author[0000-0001-6755-1315]{Joel Leja}
\PSU
\ICDS
\IGC

\author[0000-0003-3460-506X]{Shivani Bhandari}
\CSIRO

\author[0000-0002-8101-3027]{Cherie K. Day}
\Swin
\CSIRO

\author[0000-0001-9434-3837]{Adam T. Deller}
\Swin

\author[0000-0003-1913-3092]{Pravir Kumar}
\Swin

\author[0000-0002-7738-6875]{J.~Xavier~Prochaska}
\UCSC
\IPMU

\author[0000-0002-6895-4156]{Danica R. Scott}
\Curtin

\author[0000-0003-2149-0363]{Keith W. Bannister}
\CSIRO

\author[0000-0003-0307-9984]{Tarraneh Eftekhari}
\CfA

\author[0000-0002-5025-4645]{Alexa C. Gordon}
\NU

\author[0000-0002-9389-7413]{Kasper E. Heintz}
\IS\DAWN

\author{Clancy W. James}
\Curtin

\author[0000-0002-5740-7747]{Charles D. Kilpatrick}
\NU

\author[0000-0002-5053-2828]{Elizabeth K. Mahony}
\CSIRO

\author[0000-0003-3937-0618]{Alicia Rouco Escorial}
\NU

\author[0000-0003-4501-8100]{Stuart D. Ryder}
\MQ
\MQAAAstro

\author[0000-0002-7285-6348]{Ryan M. Shannon}
\Swin

\author[0000-0002-1883-4252]{Nicolas Tejos}
\PUCV

==> FRB 201124A host/tables/allproperties.tex <==
\begin{deluxetable}{ccc}[t!]
\linespread{1.2}
\tablecaption{Derived Host Galaxy Properties of \frb\ \label{tab:allprops}}
\tablecolumns{3}
\tablewidth{0pt}
\tablehead{
\colhead{Property} &
\colhead{Value} & 
\colhead{Units}
}
\startdata
$z$ & $0.0979 \pm 0.0001$ \\
RA(J2000) & \ra{5}{08}{03.477}  \\
Dec(J2000) & $+$\dec{26}{03}{37.93} \\
$\delta R$ (VLBI) & $0.71 \pm 0.03$ & $''$ \\
$\delta R$ (VLBI) & $1.29 \pm 0.05$ & kpc \\
SFR (H$\alpha$) & $2.1^{+0.7}_{-0.3}$ & $M_{\odot}$~yr$^{-1}$ \\
SFR ($3-1100\,\mu m$) & $4.0^{+0.9}_{-0.5}$ & $M_{\odot}$~yr$^{-1}$ \\
SFR (radio)$^\dagger$ & $2.2-5.9$ & $M_{\odot}$~yr$^{-1}$ \\
12$+$log(O/H) & $9.03^{+0.15}_{-0.24}$ \\
log($L_B/L_{\odot}$) & 10.10 \\
\hline
\multicolumn{3}{c}{\emph{{\tt Prospector} Parametric Fit}} \\
\hline
log(M$_*$/M$_{\odot}$) & $10.23 ^{+0.02}_{-0.03}$ \\
$t_m$ & $4.97^{+0.36}_{-0.52}$ & Gyr \\
$t_{\rm max}$ & $11.00^{+0.92}_{-1.35}$ & Gyr \\
$\tau$ & $5.62^{+0.86}_{-1.02}$ & Gyr \\
log(Z$_*$/Z$_{\odot}$) & $-0.87 \pm 0.06$ \\
log(Z$_{\rm gas}$/Z$_{\odot}$) & $0.13 \pm 0.01$ \\
$A_{\rm V, old}$ & $1.02 \pm 0.04$ & mag \\
SFR$_{\rm SED}$ & $2.43 \pm 0.13$ & $M_{\odot}$~yr$^{-1}$ \\
\hline
\multicolumn{3}{c}{\emph{{\tt Prospector} Non-Parametric Fit}} \\
\hline
log(M$_*$/M$_{\odot}$) & $10.28 \pm 0.05$ \\
$t_m$ & $6.16^{+0.75}_{-0.80}$ & Gyr \\
log(Z$_*$/Z$_{\odot}$) & $-0.58 \pm 0.22$ \\
log(Z$_{\rm gas}$/Z$_{\odot}$) & $0.17^{+0.29}_{-0.19}$ \\
$A_{V, {\rm young}}$ & $0.91^{+0.44}_{-0.39}$ & mag \\
$A_{V, {\rm old}}$ & $0.81^{+0.20}_{-0.16}$ & mag \\
SFR$_{\rm SED}^{\ddagger}$ & $1.50^{+0.52}_{-0.35}$ & $M_{\odot}$~yr$^{-1}$ \\
sSFR(100~Myr) & $1.38^{+0.75}_{-0.49}$ & $10^{-10}$~yr$^{-1}$ 
\enddata
\tablecomments{Properties of \frb\ and its host galaxy determined in this work. The {\tt Prospector} parametric fit is characterized by a MW extinction law and delayed-$\tau$ SFH. Quoted upper limits correspond to the $99.7\%$ quantile. The {\tt Prospector} property definitions are described in Section~\ref{sec:prospector} \\
$\dagger$ Range set by frequency and calibration method \citep{yc02,mcs+11}. \\
$\ddagger$ Corresponds to ongoing SFR in most recent age bin.}
\end{deluxetable}

==> FRB 201124A host/tables/frbprops.tex <==
\begin{deluxetable*}{ccccccccccccc}[!t]
\tablecaption{Properties of Three ASKAP Bursts from the \frb\ Source \label{tab:loc}}
\tablecolumns{10}
\tablewidth{0pt}
\tablehead{
\colhead{Date} &
\colhead{TNS Name} & 
\colhead{Burst No.} & 
\colhead{Frequency} & 
\colhead{Fluence} & 
\colhead{DM} & 
\colhead{RA} & 
\colhead{Decl.} &
\colhead{$\sigma_{\rm maj}$} &
\colhead{$\sigma_{\rm min}$} &
\colhead{$\sigma_{\rm PA}$}  \\
\colhead{(UT)} & 
\colhead{} &
\colhead{} &
\colhead{(MHz)} & 
\colhead{(Jy~ms)} & 
\colhead{(pc~cm$^{-3}$)} & 
\colhead{(J2000)} & 
\colhead{(J2000)} & 
\colhead{($''$)} & 
\colhead{($''$)} & 
\colhead{(deg)} 
}
\startdata
2021-04-01 & 20210401A & A02 & 864.5 & $187 \pm 12$  & $412 \pm 3$ & \ra{05}{08}{03.48} & $+$\dec{26}{03}{38.4} & 1.3 & 0.7 & 140 \\
2021-04-02 & 20210402A & A03 & 1271.5 & $22 \pm 3$ & $414 \pm 3$ & \ra{05}{08}{03.67} & $+$\dec{26}{03}{39.5} & 1.6 & 0.9 & 42 \\
2021-04-04 & 20210404B & A07 & 1271.5 & $11 \pm 2$ & $414 \pm 3$ & \ra{05}{08}{03.55} & $+$\dec{26}{03}{39.1} & 1.1 & 0.7 & 13 \\
Combined  &  & & & & & \ra{05}{08}{03.54} & $+$\dec{26}{03}{38.4} & 0.9 & 0.8 & 171   \\
\hline
\enddata
\tablecomments{Uncertainties correspond to $1\sigma$ confidence. $\sigma_{\rm maj}$ and $\sigma_{\rm min}$ are the uncertainties along the semi-major and semi-minor axes respectively, and then rotated by the $\sigma_{\rm PA}$, defined as the position angle East of North.}
\end{deluxetable*}

==> FRB 201124A host/tables/nebemline.tex <==
\begin{deluxetable}{cc}[t!]
\linespread{1.2}
\tablecaption{\frb\ Host Nebular Emission Line Fluxes \label{tab:nebemline}}
\tablecolumns{3}
\tablewidth{0pt}
\tablehead{
\colhead{Line} &
\colhead{$F_{\lambda}$} \\
\colhead{} &
\colhead{($10^{-15}$ erg s$^{-1}$ cm$^{-2}$)}
}
\startdata
H$\beta$ & $1.23^{+0.30}_{-0.23}$ \\
{[}\oiii{]} $\lambda 4959$ & $0.12^{+0.07}_{-0.03}$ \\
{[}\oiii{]}$\lambda 5007$ & $0.38^{+0.21}_{-0.11}$ \\
{[}\nii{]}$\lambda 6548$ & $0.85^{+0.20}_{-0.16}$ \\
H$\alpha$ & $5.69^{+1.49}_{-0.99}$ \\
{[}\nii{]}$\lambda 6583$ & $2.53^{+0.60}_{-0.47}$ \\
{[}\sii{]}$\lambda 6716$ & $1.08^{+0.25}_{-0.20}$ \\
{[}\sii{]}$\lambda 6731$ & $0.84^{+0.19}_{-0.15}$ \\
\enddata
\tablecomments{These values are derived from {\tt Prospector}, and are corrected for underlying stellar absorption and Galactic extinction in the direction of the host.}
\end{deluxetable}

==> FRB 201124A host/tables/photometry.tex <==
\begin{deluxetable*}{cccccc}[t!]
\linespread{1.1}
\tablecaption{\frb\ Host Galaxy Photometry \label{tab:hostphot}}
\tablecolumns{6}
\tablewidth{0pt}
\tablehead{
\colhead{Source} &
\colhead{Filter/Band} &
\colhead{$m_{\lambda}$} & 
\colhead{$A_{\lambda}$} &
\colhead{$F_{\nu}$} &
\colhead{$\nu L_{\nu}$} \\
\colhead{} &
\colhead{} &
\colhead{(AB mag)} & 
\colhead{(mag)} &
\colhead{($\mu$Jy)} &
\colhead{(erg s$^{-1}$)}
}
\startdata
{\it Swift}/XRT & 1.7~keV & - & - & $<0.0128$ & $<1.28 \times 10^{42}$ \\
SDSS & $u$ & $19.974 \pm 0.545$ & 3.075 & $37.1 \pm 24.2$ & $(7.73 \pm 0.50) \times 10^{42}$ \\
Pan-STARRS & $g$ & $18.462 \pm 0.038$ & 2.276 & $149.7 \pm 5.3$ & $(2.29 \pm 0.08) \times 10^{43}$ \\
Pan-STARRS & $r$ & $17.904 \pm 0.029$ & 1.637 & $250.2 \pm 6.8$ & $(2.99 \pm 0.08) \times 10^{43}$ \\
Pan-STARRS & $i$ & $17.591 \pm 0.034$ & 1.186 & $333.9 \pm 10.6$ & $(3.27 \pm 0.10) \times 10^{43}$ \\
Pan-STARRS & $z$ & $17.419 \pm 0.028$ & 0.920 & $391.2 \pm 10.2$ & $(3.33 \pm 0.09) \times 10^{43}$ \\
Pan-STARRS & $y$ & $17.385 \pm 0.059$ & 0.759 & $403.7 \pm 22.5$ & $(3.09 \pm 0.17) \times 10^{43}$ \\
2MASS & $J$ & $16.964 \pm 0.119$ & 0.480 & $594.5 \pm 68.9$ & $(3.50 \pm 0.41) \times 10^{43}$ \\
2MASS & $H$ & $16.787 \pm 0.123$ & 0.283 & $700.2 \pm 83.4$ & $(3.12 \pm 0.37) \times 10^{43}$ \\
2MASS & $K$ & $16.707 \pm 0.115$ & 0.171 & $753.7 \pm 84.2$ & $(2.58 \pm 0.28) \times 10^{43}$ \\
WISE & $W1$ & $17.127 \pm 0.041$ & 0.075 & $511.9 \pm 19.7$ & $(1.12 \pm 0.04) \times 10^{43}$ \\
WISE & $W2$ & $17.443 \pm 0.048$ & 0.044 & $382.7 \pm 17.3$ & $(6.10 \pm 0.27) \times 10^{42}$ \\
WISE & $W3$ & $14.998 \pm 0.061$ & 0.013 & $3637.5 \pm 210.2$ & $(2.22 \pm 0.13) \times 10^{43}$ \\
WISE & $W4$ & $14.587 \pm 0.256$ & 0.007 & $5311.3 \pm 1412.3$ & $(1.76 \pm 0.47) \times 10^{43}$  \\
uGMRT & 650~MHz & - & - & $700 \pm 100$ & $(1.12 \pm 0.16) \times 10^{38}$ \\
VLA & 1.4~GHz & - & - & $<510$ & $\lesssim 1.76 \times 10^{38}$ \\
VLA & 3~GHz & - & - & $340 \pm 30$ & $(2.51 \pm 0.22) \times 10^{38}$ \\
VLA & 6~GHz & - & - & $221 \pm 21$ & $(3.26 \pm 0.31) \times 10^{38}$ \\
VLA & 9~GHz & - & - & $150 \pm 10$ & $(3.32 \pm 0.22) \times 10^{38}$ \\
\enddata
\tablecomments{Magnitudes $m_{\lambda}$ are corrected for Galactic extinction, $A_{\lambda}$, in the direction of the burst \citep{fm07}. Data are from the {\it Swift} archive (Program~1619112), SDSS~DR12 \citep{SDSS2020}, Pan-STARRS DR1 \citep{cmm+16}, 2MASS \citep{2MASS}, and AllWISE \citep{WISE,AllWISE}. uGMRT and VLA measurements are from \citet{atel14529}, \citet{atel14549}, and \citet{rll+21}. Upper limits correspond to the estimated $3\sigma$ confidence.}
\end{deluxetable*}

==> FRB 201124A host/tables/priors.tex <==
\begin{deluxetable}{cc}[t!]
\linespread{1.2}
\tablecaption{Prior Ranges for {\tt Prospector} Fitting \label{tab:priors}}
\tablecolumns{2}
\tablewidth{0pt}
\tablehead{
\colhead{Property} &
\colhead{Range} 
}
\startdata
log(M$_F$/M$_{\odot}$) & [8, 12]  \\ 
log($r_i$) & [-100,100]$^{\ddagger}$ \\
$t_{\rm age}^{\dagger}$ (Gyr) & [0, 12.4] \\
$\tau^{\dagger}$ (Gyr) & [0.1, 10] \\
log(Z$_*$/Z$_{\odot}$) & [-2.0, 0.19] \\ 
log(Z$_{\rm gas}$/Z$_{\odot}$) & [-2, 0.5] \\
dust1/dust2 & [0, 1.5] \\ 
dust2 & [0, 4] \\ 
$f_{\rm AGN}$ & [$10^{-5}$, 3.0] \\
$\tau_{\rm AGN}$ & [5.0, 150.0] 
\enddata
\tablecomments{$\dagger$ For parametric SFH fits only. \\
$\ddagger$ For non-parametric SFH fits only.}
\end{deluxetable}
